Atmospheric pressure and molecular cloud formation in early-type galaxies

A strong correlation between atmospheric pressure and molecular gas mass is found in central cluster galaxies and early-type galaxies. This trend and a similar trend with atmospheric gas density would naturally arise if the molecular clouds condensed from hot atmospheres. Limits on the ratio of molecular to atomic hydrogen in these systems exceed unity. The data are consistent with ambient pressure being a significant factor in the rapid conversion of atomic hydrogen into molecules as found in normal spiral galaxies.

==> defn.tex <==
%-*-LaTeX-*-
% Copied from gmorris
% Note that some of these call others, eg \kmps uses \km.

% journals
%\newcommand{\apj}{ApJ}
%\newcommand{\mnras}{MNRAS}
%\newcommand{\nat}{Nat}
%\newcommand{\physrevB}{Phys. Rev. B}
%\newcommand{\araa}{ARA\&A}                % "Ann. Rev. Astron. Astrophys."
%\newcommand{\aap}{A\&A}                   % "Astron. Astrophys."
%\newcommand{\aaps}{A\&AS}                 % "Astron. Astrophys. Suppl. Ser."
%\newcommand{\aj}{AJ}                      % "Astron. J."
%\newcommand{\apjs}{ApJS}                  % "Astrophys. J. Suppl. Ser."
%\newcommand{\pasp}{PASP}                  % "Publ. Astron. Soc. Pac."
%\newcommand{\apjl}{ApJ}                   % letter at ApJ
%\newcommand{\pasj}{PASJ}
%\newcommand{\gca}{Geochim. Cosmochim. Acta}
%\newcommand{\physrep}{Phys. Rep.}
%\newcommand{\aapr}{A\&A Rev.}
%\newcommand{\ssr}{Space Sci. Rev.}
%\newcommand{\na}{New Astron.}
%\newcommand{\nar}{NewA Rev.}
%\newcommand{\jgr}{J. Geophys. Res.}

% Length
\newcommand{\Mpc}{\rm\; Mpc}
\newcommand{\kpc}{\rm\; kpc}
\newcommand{\pc}{\rm\; pc}
\newcommand{\km}{\rm\; km}
\newcommand{\m}{\rm\; m}
\newcommand{\cm}{\rm\; cm}
\newcommand{\mum}{\hbox{$\rm\; \mu m\,$}}
\newcommand{\pix}{\rm\; pixel}
%
\newcommand{\cmps}{\hbox{$\cm\s^{-1}\,$}}
\newcommand{\cmpssq}{\hbox{$\cm\s^{-2}\,$}}
\newcommand{\cmsq}{\hbox{$\cm^2\,$}}
\newcommand{\cmcu}{\hbox{$\cm^3\,$}}
\newcommand{\pcmcuK}{\hbox{$\cm^{-3}\K\,$}}
\newcommand{\ppix}{\hbox{$\pix^{-1}\,$}}
\newcommand{\ppixsq}{\hbox{$\pix^{-2}\,$}}
\newcommand{\kpcsq}{\hbox{$\kpc^{2}\,$}}
% Length


% Time
\newcommand{\hr}{\rm\; hr}
\newcommand{\yr}{\rm\; yr}
\newcommand{\Gyr}{\rm\; Gyr}
\newcommand{\Myr}{\rm\; Myr}
\newcommand{\s}{\rm\; s}
\newcommand{\ms}{\rm\; ms}
\newcommand{\ks}{\rm\; ks}
\newcommand{\mus}{\hbox{$\rm\; \mu s\,$}}
% Time


% Frequency
\newcommand{\GHz}{\rm\; GHz}
\newcommand{\MHz}{\rm\; MHz}
\newcommand{\Hz}{\rm\; Hz}
% Frequency


% Temperature
\newcommand{\K}{\rm\; K}
% Temperature


% Pressure
\newcommand{\Kpcmc}{\hbox{$\K\cm^{-3}\,$}}
\newcommand{\keVpcmcu}{\hbox{$\keV\cm^{-3}\,$}}
% Pressure


% Mass
\newcommand{\g}{\rm\; g}
%
\newcommand{\gpcm}{\hbox{$\g\cm^{-3}\,$}}
\newcommand{\gpcmps}{\hbox{$\g\cm^{-3}\s^{-1}\,$}}
\newcommand{\gps}{\hbox{$\g\s^{-1}\,$}}
%
\newcommand{\Msun}{\hbox{$\rm\thinspace M_{\odot}$}}
\newcommand{\Msunpc}{\hbox{$\Msun\pc^{-3}\,$}}
\newcommand{\Msunpkpc}{\hbox{$\Msun\kpc^{-1}\,$}}
\newcommand{\Msunppc}{\hbox{$\Msun\pc^{-3}\,$}}
\newcommand{\Msunppcpyr}{\hbox{$\Msun\pc^{-3}\yr^{-1}\,$}}
\newcommand{\Msunpyr}{\hbox{$\Msun\yr^{-1}\,$}}
% Mass


% Energy
\newcommand{\MeV}{\rm\; MeV}
\newcommand{\keV}{\rm\; keV}
\newcommand{\eV}{\rm\; eV}
\newcommand{\erg}{\rm\; erg}
\newcommand{\Jy}{\rm\; Jy}
\newcommand{\mJy}{\rm\; mJy}
\newcommand{\W}{\rm\; W}
%
\newcommand{\ergcmcups}{\hbox{$\erg\cm^3\ps\,$}}
\newcommand{\ergpcmps}{\hbox{$\erg\cm^{-3}\s^{-1}\,$}}
\newcommand{\ergpcmsq}{\hbox{$\erg\cm^{-2}\,$}}
\newcommand{\ergpcmcu}{\hbox{$\erg\cm^{-3}\,$}}
\newcommand{\ergpcmsqps}{\hbox{$\erg\cm^{-2}\s^{-1}\,$}}
\newcommand{\ergpcmsqpspA}{\hbox{$\erg\cm^{-2}\s^{-1}$\AA$^{-1}\,$}}
\newcommand{\ergpcmsqpspsr}{\hbox{$\erg\cm^{-2}\s^{-1}\sr^{-1}\,$}}
\newcommand{\ergpcmcups}{\hbox{$\erg\cm^{-3}\s^{-1}\,$}}
\newcommand{\ergps}{\hbox{$\erg\s^{-1}\,$}}
\newcommand{\ergpspHz}{\hbox{$\erg\s^{-1}\pHz\,$}}
\newcommand{\ergpspmp}{\hbox{$\erg\s^{-1}\Mpc^{-3}\,$}}
\newcommand{\ergpspkpc}{\hbox{$\erg\s^{-1}\kpc^{-1}\,$}}
%
\newcommand{\keVpcmsqpspsr}{\hbox{$\keV\cm^{-2}\s^{-1}\sr^{-1}\,$}}
%
\newcommand{\WpHzpsr}{\hbox{$\W\pHz\psr\,$}}
\newcommand{\WpHz}{\hbox{$\W\pHz\,$}}
%
\newcommand{\surbri}{\hbox{$\rm\thinspace photons\pcmsq\ps\pasecsq$}}
\newcommand{\expmapcorr}{\hbox{$\rm\thinspace photons\pcmsq\ps\ppix$}}
% Energy


% Force
\newcommand{\dyn}{\rm\; dyn}
\newcommand{\dynpcmsq}{\hbox{$\dyn\cm^{-2}\,$}}
% Force


% Speed
\newcommand{\kmps}{\hbox{$\km\s^{-1}\,$}}
\newcommand{\kmpspmp}{\hbox{$\km\s^{-1}\Mpc{-1}\,$}}
\newcommand{\kmpspMpc}{\hbox{$\kmps\Mpc^{-1}\,$}}
% Speed


% Luminosity
\newcommand{\Lsun}{\hbox{$\rm\thinspace L_{\odot}$}}
\newcommand{\Lsunppc}{\hbox{$\Lsun\pc^{-3}\,$}}
% Luminosity


% Misc
\newcommand{\dex}{\rm\; dex}

\newcommand{\plawnorm}{\hbox{$\rm\thinspace photons\keV^{-1}\cm^{-2}\s^{-1}\,$}}
\newcommand{\Zsun}{\hbox{$\thinspace \mathrm{Z}_{\odot}$}}

\newcommand{\gauss}{\rm\; gauss}
\newcommand{\muG}{\hbox{$\rm\thinspace {\mu}\mathrm{G}$}}
%
\newcommand{\chisq}{\hbox{$\chi^2$}}
\newcommand{\delchi}{\hbox{$\Delta\chi$}}
%
\newcommand{\ph}{\rm\; ph}
% Misc

% Angles
\newcommand{\amin}{\rm\; arcmin}
\newcommand{\aminsq}{\hbox{$\amin^{2}\,$}}
\newcommand{\asec}{\rm\; arcsec}
\newcommand{\asecsq}{\hbox{$\asec^{2}\,$}}
\newcommand{\sr}{\rm\; sr}
\newcommand{\degword}{\rm\; deg}
\newcommand{\degsq}{\hbox{$\degword^2\,$}}
% Angles

% Emission measure
\newcommand{\emm}{\hbox{$\cm^{-5}\,$}}
\newcommand{\sqremm}{\hbox{$\cm^{-5/2}\,$}}
\newcommand{\empasecsq}{\hbox{$\emm\asec^{-2}\,$}}
\newcommand{\keVempasecsq}{\hbox{$\keV\emm\asec^{-2}\,$}}
\newcommand{\pseudoP}{\hbox{$\keV\sqremm\asec^{-2}\,$}}
% Emission measure

% Per something
\newcommand{\pcm}{\hbox{$\cm^{-1}\,$}}
\newcommand{\psqcm}{\hbox{$\cm^{-2}\,$}}
\newcommand{\pcmsq}{\hbox{$\cm^{-2}\,$}}
\newcommand{\pcmcu}{\hbox{$\cm^{-3}\,$}}
\newcommand{\pcmcus}{\hbox{$\pcmcu\s\,$}}
\newcommand{\pmpc}{\hbox{$\Mpc^{-1}\,$}}
\newcommand{\pmpccu}{\hbox{$\Mpc^{-3}\,$}}
\newcommand{\ps}{\hbox{$\s^{-1}\,$}}
\newcommand{\pHz}{\hbox{$\Hz^{-1}\,$}}
\newcommand{\pcmK}{\hbox{$\cm^{-3}\K$}}
\newcommand{\phpcmsqps}{\hbox{$\ph\cm^{-2}\s^{-1}\,$}}
\newcommand{\psr}{\hbox{$\sr^{-1}\,$}}
\newcommand{\pasecsq}{\hbox{$\asec^{-2}\,$}}
% Per something

% Use times for maths fonts
% \DeclareSymbolFont{operators}   {OT1}{ptmcm}{m}{n}
% \DeclareSymbolFont{letters}     {OML}{ptmcm}{m}{it}
% \SetMathAlphabet{\mathbf}{normal}{\encodingdefault}{\rmdefault}{\bfdefault}{n}%
% \SetMathAlphabet{\mathsf}{normal}{\encodingdefault}{\sfdefault}{m}{n}%
% \SetMathAlphabet{\mathrm}{normal}{\encodingdefault}{\rmdefault}{m}{n}%
% \SetSymbolFont{operators}{bold}{OT1}{ptmcm}{b}{n}
% \SetSymbolFont{letters}{bold}{OML}{ptmcm}{b}{it}
% \SetMathAlphabet{\mathbf}{bold}{\encodingdefault}{\rmdefault}{m}{n}%
% \SetMathAlphabet{\mathsf}{bold}{\encodingdefault}{\sfdefault}{b}{n}%
% \SetMathAlphabet{\mathrm}{bold}{\encodingdefault}{\rmdefault}{b}{n}%

%\thinmuskip=2.5mu
%\medmuskip=3.5mu plus 1mu minus 1mu
%\thickmuskip=4.5mu plus 1.5mu minus 1mu
%\DeclareSymbolFont{symbols}     {OMS}{cmsy}{m}{n}
%\DeclareSymbolFont{largesymbols}{OMX}{cmex}{m}{n}
%\SetSymbolFont{symbols}{bold}{OMS}{cmsy}{b}{n}
%\SetSymbolFont{largesymbols}{bold}{OMX}{cmex}{m}{n}

